Hereditary Categories with Serre Duality which are generated by Preprojectives

We show that every k-linear abelian Ext-finite hereditary category with Serre duality which is generated by preprojective objects is derived equivalent to the category of representations of a strongly locally finite thread quiver.

==> SemiHereditary.tex <==

\renewcommand{\r}{\to}  

  
\section{Semi-hereditary dualizing $k$-varieties}\label{section:SemiHereditary}

\subsection{Preadditive semi-hereditary categories}

We say that a small preadditive category $\frak{a}$ is \emph{semi-hereditary}\index{category!semi-hereditary} if the finitely presented objects $\mod(\frak{a})$ in $\Mod(\frak{a})$ form an abelian and hereditary category.  The following proposition (\cite{vanRoosmalen06}, see also\cite[Theroem 1.6]{AuslanderReiten75}) shows that semi-hereditariness is a local property.

\begin{proposition}\label{proposition:ShIsLocal}
Let $\frak{a}$ be a small preadditive category, then $\frak{a}$ is semi-hereditary if and only if any full subcategory of $\frak{a}$ with a finite number of objects is semi-hereditary.
\end{proposition}

\begin{lemma} Let $\frak{b}\to \frak{c}$ be a full embedding of
  preadditive categories. Then
  $\frak{c}\otimes_{\frak{b}}-:\mod(\frak{b})\to \mod(\frak{c})$ is
  fully faithful.
\end{lemma}

\begin{proof} This may be checked on objects of the form 
$\frak{b}(-,B)$ where it is clear. 
\end{proof}

Since $(\frak{c}\otimes_{\frak{b}}-,(-)_{\frak{b}})$ is an adjoint pair, if follows from this lemma that $(\frak{c}\otimes_{\frak{b}}-)_{\frak{b}}$ is naturally isomorphic to the identity functor on $\mod(\frak{b})$.

The following result is a slight generalization of \cite[Proposition 2.2]{AuslanderReiten75}.
  
\begin{proposition}
\label{proposition:SemiHereditaryExact}
Let $\frak{b}\to \frak{c}$ be a full embedding of semi-hereditary categories. 
Then the (fully faithful) functor $\frak{c}\otimes_{\frak{b}}-:\mod(\frak{b})\to \mod(\frak{c})$
is exact.
\end{proposition}

\begin{proof}
  Let $M\in \mod(\frak{b})$ and consider a projective resolution $0\r
  P_1\xrightarrow{\theta} P_0 \r M\r 0$ in $\mod(\frak{b})$. Then
  $P_1$ is a direct summand of some $\oplus_{i=1}^n\frak{b}(-,B_i)$.
  Put $K=\ker(\frak{c}\otimes_{\frak{b}}\theta)$. Then $K$ is a direct
  summand of $\frak{c}\otimes_{\frak{b}}P_1$ (since $\frak{c}$ is semi-hereditary) and
  $K_{\frak{b}}=0$ (since $\theta$ is injective).

Assume $K$ is
  non-zero. Since $K$ is a direct summand of $\frak{c}\otimes_{\frak{b}}P_1$ we obtain a non-zero map $\frak{c}\otimes_{\frak{b}}P_1\r
K$ and hence a non-zero map $\oplus_{i=1}^n\frak{c}(-,B_i)\r K$ and
thus ultimately a non-zero element of some $K(B_i)$, contradicting the
fact that $K_{\frak{b}}=0$.

Thus $K=0$. If we denote the left satellites of $\frak{c}\otimes_{\frak{b}}-$
by $\Tor_i^{\frak{b}}(\frak{c},-)$ then we have just shown that
$\Tor_i^{\frak{b}}(\frak{c},-)=0$ for $i>0$. Hence $\frak{c}\otimes_{\frak{b}}-$
is exact. 
\end{proof}

\subsection{Dualizing $k$-varieties}\label{section:Dualizing}

We now recall some definitions from \cite{AuslanderReiten74}.  A Hom-finite additive $k$-linear category where idempotents split is called a \emph{finite $k$-variety}\index{k-variety@$k$-variety!finite}.  Note that a finite $k$-variety is always Krull-Schmidt.

Let $\frak{a}$ be a finite $k$-variety.  There is a functor $D
\colon \Fun(\frak{a}, \mod k) \to \Fun(\frak{a}^{\circ}, \mod k)$
given by sending a module $M \colon \frak{a} \to \mod k$ to the dual
$D(M)$ where $D(M)(x) = \Hom_k(M(x), k)$ for all $x \in \frak{a}$.
If this functor induces a duality $D \colon \mod \frak{a} \to \mod
\frak{a}^{\circ}$ by restricting to the finitely presented objects
in $\Fun(\frak{a}, \mod k) \subset \Mod \frak{a}$, then we will say
that $\frak{a}$ is a \emph{dualizing $k$-variety}\index{k-variety@$k$-variety!dualizing}.

We have the following easy proposition.

\begin{proposition}\label{proposition:Dualizing}
Let $\frak{a}$ be a finite $k$-variety, then $\frak{a}$ is a
dualizing $k$-variety if and only if all standard projectives are
cofinitely presented and all standard injectives are finitely
presented.
\end{proposition}

\begin{corollary}\label{corollary:DualizingCoherent}
A dualizing $k$-variety is coherent.
\end{corollary}

\begin{proof}
By Proposition \ref{proposition:Dualizing} the category of finitely presented representations and cofinitely presented representations coincide as subcategories of $\Mod \aa$.  The former is closed under cokernels, the latter under kernels.  This shows that $\mod \aa$ is an abelian subcategory of $\Mod \aa$.
\end{proof}

The next theorem is the main result of this section.  The main ideas of the proof are taken from \cite{ReVdB02}.

\begin{theorem}\label{theorem:RepSerreDuality}
Let $\frak{a}$ be a finite $k$-variety, then $\AA = \mod \frak{a}$ has Serre duality if and only if $\frak{a}$ is a dualizing $k$-variety and every object of $\mod \fa$ has finite projective dimension.
\end{theorem}

\begin{proof}
First, we assume $\mod \fa$ has Serre duality.  For $A,B \in \Ob \mod \fa$, we have $\Ext^i_\AA(A,B) \cong \Hom_{\Db \AA}(A,B[i]) \cong \Hom_{\Db \AA}(B[i],FA)^*$ such that $\Ext^i_\AA(A,-)$ can only be nonzero for finitely many $i$'s.  This shows that every object has finite projective dimension.

Denote by $\PP$ and $\II$ the full subcategories spanned by (standard) projective and injective objects in $\mod \aa$, respectively.  Note that for every $A,B \in \Ob \aa$, there is a natural isomorphism
$$\Hom_\AA(\aa(-,A), \aa(-,B)) \cong \Hom_\AA(\aa(A,-)^*,\aa(B,-)^*)$$
since they are, by Yoneda's lemma, both naturally isomorphic to $\aa(A,B)$, such that the Nakayama functor $N: \PP \to \II$ given by $N \aa(-,A) = \aa(A,-)^*$ is an equivalence of categories.  This lifts to an equivalence $N: \Kb \PP \to \Kb \II$.  The composition
$$\Db \AA \cong \Kb \PP \stackrel{N}{\longrightarrow} \Kb \II \to \Db \AA$$
gives the Serre functor, and is thus an equivalence.  This yields $\Kb \II \to \Db \AA$ is an equivalence and, as such, every object of $\AA$ is cofinitely presented.

For the other direction, assume $\fa$ is a dualizing $k$-variety.  Again, denote by $\PP$ and $\II$ the full subcategories spanned by (standard) projective and injective objects in $\mod \aa$, and by $N: \Kb \PP \to \Kb \II$ the equivalence induced by the Nakayama functor.  We denote the composition
$$\Db \mod \aa \cong \Kb \PP \stackrel{N}{\longrightarrow} \Kb \II \cong \Db \mod \aa$$
by $F$.

Since every $X,Y \in \Db \mod \aa$ correspond to bounded complexes of projectives in $\Kb \PP$, we may reduce to the case where $X \cong \aa(-,A)$ and $Y \cong \aa(-,B)$.  Here, the required isomorphism
$$\Hom(\aa(-,A),\aa(-,B)) \cong \Hom(\aa(-,B), \aa(A,-)^*)^*$$
follows from Yoneda's lemma.
\end{proof}

\begin{remark}
The following example shows that there are dualizing $k$-varieties $\aa$ such that $\mod \aa$ has infinite global dimension but $\mod \aa$ still has Serre duality.
\end{remark}

\begin{example}
Let $Q$ be an $A_\infty$ quiver with zig-zag orientation where every zig has one more arrow than the preceding zag, labeled as in Figure \ref{fig:ZigZag}.  We define a relation on $Q$ by requiring the composition of any two arrows to be zero.  The associated additive category $\bb$ is a dualizing $k$-variety by Proposition \ref{proposition:Dualizing}.  Since every object has finite projective dimension, Theorem \ref{theorem:RepSerreDuality} yields that $\mod \bb$ has Serre duality.  However, denoting by $S(v)$ the simple representation associated with the vertex $v \in Q$, we see that the projective dimension of $a^i_i$ is $i$ so that the global dimension of $\mod \bb$ is infinite.
\end{example}

\begin{figure}[tbh]
$$\xymatrix@=10pt{{a^1_0} \ar[rd] && {b^1_0 = a^2_0} \ar[ld] \ar[rd]&&&& {b^2_0 = a^3_0} \ar[dl] \ar[dr] \\
& {a^1_1 = b^1_1} && {a^2_1} \ar[rd] && {b^2_1}\ar[ld]&& {a^3_1} \ar[dr]\\
&&&& {a^2_2 = b^2_2} &&&& {a^3_2} \ar[dr] && \ar@{..}[dl]\\
&&&&&&&&& {a^3_3 = b^3_3}}$$
\caption{}
\label{fig:ZigZag}
\end{figure}

\begin{remark}
The category $\mod \bb$ is piecewise hereditary.  Indeed, let $\aa = kQ$, then one may define a functor by
\begin{eqnarray*}
i: \aa &\to& \ind \Db \mod \bb \\
a^i_j &\mapsto& S(a^i_j)[-j] \\
b^i_j &\mapsto& S(b^i_j)[-j]
\end{eqnarray*}
The essential image of $i$ forms a partial tilting set in $\Db \mod \bb$ which furthermore generates $\Db \mod \bb$ as a triangulated category, hence $i$ lifts to an equivalence $\Db \mod \aa \to \Db \mod \bb$ of triangulated categories.
\end{remark}

\begin{example}
Let $Q$ be an $A_\infty^\infty$ quiver with linear orientation.  We put a relation on $Q$ by requiring that the composition of any two arrows is zero.  The associated category $kQ$ is a clearly a finite $k$-variety and, since the indecomposable projectives and indecomposable injectives in $\mod kQ$ coincide, Proposition \ref{proposition:Dualizing} yields $kQ$ is a dualizing $k$-variety.

It is easy to check $\mod kQ$ has left and right almost split sequences, but Theorem \ref{theorem:RepSerreDuality} shows that $\Db \mod kQ$ has no Serre functor since every standard simple representation has infinite projective dimension.
\end{example}

\subsection{Threads}

We will say a finite $k$-variety $\aa$ is \emph{locally finite and locally discrete} if, for all $A \in \ind \aa$, there is a right almost split map $A \to M$ and a left almost split map $N \to A$, for certain objects $M,N \in \Ob \aa$.  In particular, every nonsplit map $A \to B$ or $B \to A$ factors through $A \to M$ or $N \to A$, repsectively.


\begin{example}
Let $Q$ be a finite quiver.  The path category $kQ$ is locally discrete and locally finite.
\end{example}

\begin{example}
Let $\PP$ be the poset $\bN \cdot \{+ \infty\}$.  We may draw the Auslander-Reiten quiver of $k\PP$ as
$$\xymatrix{
0 \ar[r] & 1 \ar[r] & 2 \ar[r] & 3 \ar@{..}[r]& {+\infty}
}$$
It is clear that $k\PP$ is not locally discrete.
\end{example}

We now give an equivalent formulation of these properties.

\begin{proposition}\label{proposition:LocallyFinite}
A finite $k$-variety is locally finite and locally discrete if and only if all standard simples of $\aa$ are finitely presented and cofinitely presented.  Every dualizing $k$-variety is locally finite and locally discrete.
\end{proposition}

\begin{proof}
Assume $\aa$ is locally finite and locally discrete.  For an indecomposable $A \in \ind \aa$, let $N \to A$ be a left almost split map which gives rise to a map in $\mod \aa$
$$\aa(-,N) \longrightarrow \aa(-,A).$$
It is straightforward to see that the cokernel is the standard simple $S_A$.  Dually, one shows all standard simples are cofinitely presented.

Next, assume all standard simples are finitely and cofinitely presented.  We prove that every indecomposable $A \in \ind \aa$ admits a left almost split map $N \to A$, for a certain object $N \in \Ob \aa$.  Consider a presentation of $S_A$
$$Q \longrightarrow \aa(-,A) \longrightarrow S_A \longrightarrow 0.$$
We may write the projective $Q$ as $\aa(-,N)$, and the induced map $N \to A$ is easily seen to be left almost split.

Dually, one proves a $A$ admits a right almost split map $A \to M$.

For the last part, let $\aa$ be a dualizing $k$-variety and $X \in \ind \aa$.  The associated simple representation $T_X$ is the image of $\aa(-,X) \to \aa(X,-)^*$.
\end{proof}

\begin{proposition}\label{proposition:DualizingIfLeftAndRightAdjoint}
Let $\aa$ be a dualizing $k$-variety and let $i:\bb \to \aa$ is a full embedding admitting a left adjoint $i_L$ and a right adjoint $i_R$, then $\bb$ is also a dualizing $k$-variety.
\end{proposition}

\begin{proof}
Let $X \in \Ob \bb$ and let $\aa(-,Y_2) \to \aa(-,Y_1) \to \aa(iX,-)^* \to 0$ be projective resolution in $\mod \aa$, then $\bb(-,i_R Y_2) \to \bb(-,i_R Y_1) \to \bb(X,-)^* \to 0$ is a projective resolution in $\mod \bb$.  This show that every standard injective in $\mod \bb$ is finitely presented.  Likewise, one shows that every (standard) projective in $\bb$ is cofinitely presented.  The required result follows from Proposition \ref{proposition:Dualizing}.
\end{proof}

The previous proposition will often be combined with the following result.

\begin{proposition}\label{proposition:WhenAdjoints}
Let $\aa$ be a semi-hereditary dualizing $k$-variety.  
\begin{enumerate}
\item Let $I$ be a set and $\{Z_i\}_{i \in I}$ be a set of objects of $\mod \aa$ such that $\sum_i \dim \aa(A,Z_i) < \infty$ and $\sum_i \dim \aa(Z_i,A) < \infty$ for all $A \in \Ob \aa$ and define a full subcategory $\bb$ of $\aa$ given by 
$$B \in \bb \Longleftrightarrow \forall i \in I: \Hom(\aa(-,B),Z_i) = 0.$$
The embedding $i: \bb \to \aa$ has a left and right adjoint.
\item Let $Y \in \ind \aa$.  The embedding $\supp (-,Y) \to \aa$ has a left and a right adjoint.
\item Let $X,Y \in \ind \aa$.  The embedding $[X,Y] \to \aa$ has a left and a right adjoint.
\end{enumerate}
\end{proposition}

\begin{proof}
\begin{enumerate}
\item
We start by defining the left adjoint $i_L: \aa \to \bb$.  Let $A_1 \to A_2$ be a map in $\aa$ and consider the following commutative diagram with exact rows
$$\xymatrix{
0 \ar[r] & \aa(-,A_1') \ar[r]\ar@{-->}[d] & \aa(-,A_1) \ar[r]\ar[d] & \bigoplus_i \Hom(\aa(-,A_1), Z_i)^* \otimes_k Z_i \ar[d] \\
0 \ar[r] & \aa(-,A_2') \ar[r] & \aa(-,A_2) \ar[r] & \bigoplus_i \Hom(\aa(-,A_2), Z_i)^* \otimes_k Z_i
}$$
Note that the conditions in the statement of the lemma imply that both $\bigoplus_i \Hom(\aa(-,A_1), Z_i)^* \otimes_k Z_i$ and $\bigoplus_i \Hom(\aa(-,A_2), Z_i)^* \otimes_k Z_i$ lie in $\mod \aa$.

Since both the kernel, the Yoneda embedding, and the tensor product are functorial, it is easy to see that the correspondence from $A_1 \to A_2$ to $A_1' \to A_2'$ is functorial.  It is readily checked that this functor is left adjoint to the embedding.

The right adjoint is defined in a dual way.


\item
Let $A \to B$ be a map in $\aa$.  The following commutative diagram
$$\xymatrix{
\aa(-,A) \ar[rr]^-f \ar[rd] \ar[ddd]&& \aa(-,Y) \otimes \Hom(A,Y)^* \ar[ddd] \\
&\im f \ar[ru] \ar@{-->}[d] \\
&\im g \ar[rd] \\
\aa(-,B) \ar[rr]^-g \ar[ru] && \aa(-,Y) \otimes \Hom(B,Y)^*
}$$
gives a map $\im f \to \im g$.  Since $\mod \aa$ is hereditary, both $\im f$ and $\im g$ are projective and hence of the form $\aa(-,A')$ and $\aa(-,B')$, respectively.  The objects $A'$ and $B'$ lie in $\supp \aa(-,Y)$ and the correspondence $A \to B$ to $A' \to B'$ is functorial.  It is readily checked that this defines a left adjoint $i_L: \aa \to \supp \aa(-,Y)$ to the functor $i$.

To find is a right adjoint, it suffices to show that every functor of the form $\aa(i-,X)$ is representable or, equivalently, a finitely generated projective object in $\Mod \bb$.  Let $M \to \aa(i-,X)$ be an epimorphism in $\Mod \bb$.  Applying $\aa \otimes_\bb -$ and using that $i$ is fully faithful gives an epimorphism
$$\aa \otimes_\bb M \to \aa(-,X)$$
which is split.  Applying the restriction to $\bb$ gives that $M \to \aa(i-,X)$ is split (here we use that $(\aa \otimes_bb -)_\bb$ is the identity), thus $\aa(i-,X)$ is a projective object in $\Mod \bb$.  Since $\aa \otimes_\bb \aa(i-,X)$ is a finitely generated projective object, so is $\aa(i-,X)$.  This shows $i: \supp (-,Y) \to \aa$ admits a right adjoint.

\item 
Propositions \ref{proposition:ShIsLocal} and \ref{proposition:DualizingIfLeftAndRightAdjoint} imply that $\supp \aa(-,Y)$ is a semi-hereditary dualizing $k$-variety.  The requested result now follows easily from the dual of the previous result.
\end{enumerate}
\end{proof}

We now come to the definition of threads.

\begin{definition}
If $\aa$ is a semi-hereditary dualizing $k$-variety, a locally finite and locally discrete object $X \in \ind \aa$ will be called a \emph{thread object}\index{thread!object} if $X$ has a unique direct predecessor and a unique direct successor, or equivalently, there is a right almost split map $X \to M$ and a left almost split map $N \to X$ where $M$ and $N$ are indecomposable.  In this case, we will denote the representatives of $M$ and $N$ in $\ind \aa$ by $X^+$ and $X^-$, respectively.

For $X,Y \in \ind \aa$, the interval $[X,Y]$ will be called a \emph{thread} if every indecomposable object is a thread object.

An indecomposable object that is not a thread object is called a \emph{non-thread object}\index{non-thread object}.
\end{definition}

\begin{proposition}\label{propostition:ThreadsInVarieties}
Let $\aa$ be a semi-hereditary dualizing $k$-variety, and $X,Y,Z \in \ind \aa$, then
\begin{enumerate}
\item $\supp \aa(X,-)$ and $\supp \aa(-,X)^*$ have only finitely many non-thread objects.
\item if $[X,Y]$ is a thread, then $\dim \aa(X,Y) = 1$, and
\item if $[X,Y]$ and $[X,Z]$ are threads, then either $[X,Y] \subseteq [X,Z]$ or $[X,Z] \subseteq [X,Y]$.
\end{enumerate}
\end{proposition}

\begin{proof}
\begin{enumerate}
\item It follows from Proposition \ref{proposition:Dualizing} that $\aa(X,-)$ is cofinitely presented.  Since $\aa$ is semi-hereditary, we see that $\supp \aa(X,-)$ has only finitely many non-thread objects.  The other case is dual.

\item Write $V = \aa(X,Y)$ and consider the canonical map $\aa(-,Y) \otimes_k V \to \aa(X,-)^*$ with image $F \in \mod \aa$.  We have the following short exact sequences
\begin{equation}\label{equation:TheadSequence1}
\xymatrix@1{0 \ar[r] & \aa(-,A) \ar[r] & \aa(-,Y) \otimes V \ar[r] & F \ar[r] & 0}
\end{equation}
\begin{equation}\label{equation:TheadSequence2}
\xymatrix@1{0 \ar[r] & F \ar[r] & \aa(X,-)^* \ar[r] & \aa(B,-)^* \ar[r] & 0}
\end{equation}
It is clear that every direct summand of $A$ maps nonzero to $Y$.  Furthermore, from the second short exact sequence we obtain $\dim F(X) = 1$ so that $\dim V > 1$ would imply $\dim \aa(X,A) \not= 0$.  Thus at least one indecomposable direct summand $A_1$ of $A$ lies in $[X,Y[$, hence $A_1$ is a thread object with direct successor $A_1^+ \in ]X,Y] \subset \ind \aa$.  Note that $\dim F(A_1) < \dim F(A_1^+)$.

However, applying $\aa(-,Y)$ to the sequence (\ref{equation:TheadSequence2}) yields $\aa(B,Y) = 0$.  In particular, for every $Z \in [X,Y]$, we have $\dim \aa(B,Z) = 0$ and thus $\dim F(Z) = \dim \aa(X,Z)$.  We find $\dim \aa(X,A_1) < \dim \aa(X,A_1^+)$, a contradiction since $\aa$ is semi-hereditary.

\item Let $i: [X,Y] \to \aa$ be the natural embedding.  By Proposition \ref{proposition:HasAdjoints} we know that the embedding has a right adjoint $i_R: \aa \to [X,Y]$.  Let $A$ be an indecomposable direct summand of $i_R(Z)$; since $\aa(Y,Z) = 0$, we know $A \not\cong Y$ such that $A^+ \in \Ob [X,Y]$.

Since $A \to A^+$ is left and right almost split, we know that $\dim \aa(iA,Z) = \dim \aa(iA^+,Z)$, but from the choice of $A$, we obtain $\dim \aa(A,i_R Z) > \dim \aa(A^+,i_R Z)$, a contradiction.
\end{enumerate}
\end{proof}

\begin{corollary}\label{corollary:ThreadsPosets}
Let $\aa$ be a semi-hereditary dualizing $k$-variety and let $\bb$ be the full subcategory of $\aa$ with $\Ob \bb = [X,Y]$, then $\bb \cong k \LL$ for a linearly ordered locally discrete poset $\LL$ with a maximal and a minimal element.
\end{corollary}

\begin{proof}
Let $\LL = [X,Y]$.  We define a poset structure on $\LL$ by
$$A \leq B \Longleftrightarrow \aa(A,B) \not= 0.$$
It is clear this defines a linearly ordered locally discrete poset $\LL, \leq$ with unique minimal and maximal element.  We will define a functor $k \LL \to \bb$ as follows.  For every $A \in [X,Y]$, choose a nonzero element $b_{X,A} \in \aa (X,A)$.

For every $A,B \in \ind \bb$ with $\bb(A,B) \not= 0$, this gives a unique element $b_{A,B} \in \bb(A,B)$ with $b_{X,B} = b_{X,A} \circ b_{A,B}$.

It is now easy to see that the functor $\LL \to \bb$, which is the identity on objects and sending $(A,B) \in \LL(A,B)$ to $b_{A,B} \in \bb(A,B)$, is an equivalence.
\end{proof}

\begin{corollary}
A connected semi-hereditary dualizing $k$-variety has only countably many sinks or sources.
\end{corollary}

\subsection{Thread quivers}\label{subsection:DualizingThreadQuiver}

\begin{proposition}\label{proposition:PathCategory}
Let $\aa$ be a semi-hereditary dualizing $k$-variety such that $[X,Y]$ is finite for all $X,Y \in \ind \aa$.  Write $Q$ for the Auslander-Reiten quiver of $\aa$, then $\aa$ is equivalent to $kQ$.  Moreover, $Q$ is a strongly locally finite quiver.
\end{proposition}

\begin{proof}
  For every two indecomposables $A,B \in \ind \aa$, we will choose $\dim_k \Irr(A,B)$ linearly independant irreducible maps $A \to B$.  This gives a map $f: Q_0 \to \Mor \aa$, mapping the arrows in $Q$ to the chosen irreducible maps in $\aa$.

  Let $A,B \in \ind \aa$.  Since every interval $[A,B]$ is assumed to be finite, every map $A \to B$ is a linear combination of compositions of chosen irreducible maps.
  
  There is an obvious map $F:\Ob kQ \to \Ob \aa$, which is essentially surjective since $\aa$ is Krull-Schmidt.
\end{proof}

The previous proposition does not hold without the assumption on the intervals $[X,Y]$.  However, in the case of dualizing $k$-varieties, these intervals are nicely behaved (Proposition \ref{propostition:ThreadsInVarieties}) such that an analogue of Proposition \ref{proposition:PathCategory} may be proven without any assumption on the intervals $[X,Y]$, by replacing the quiver $Q$ by a thread quiver.

A \emph{thread quiver} consists of the following information:
\begin{itemize}
\item A quiver $Q=(Q_0,Q_1)$ where $Q_0$ is the set of vertices and $Q_1$ is the set of arrows.
\item A decomposition $Q_1 = Q_s \coprod Q_t$.  Arrows in $Q_s$ will be called \emph{standard arrows}, while arrows in $Q_t$ will be referred to as \emph{thread arrows}.
\item With every thread arrow $\alpha$, there is an associated linearly ordered set $\TT_\alpha$, possibly empty.
\end{itemize}

In drawing a thread quiver (cf. Figure \ref{fig:ThreadQuiver}), standard arrows will be represented by $\xymatrix@1{\bullet \ar[r]& \bullet}$, while thread arrows will be drawn as $\xymatrix@1{\bullet\ar@{-->}[r]&\bullet}$ labeled by the corresponding ordered set $\TT$.  If $\TT = \{1,2,3, \ldots, n\}$ with the normal ordering, then we will only write $n$ as a label; if $\TT = \emptyset$, then no label will be written.

\begin{figure}\label{fig:ThreadQuiver}
$$\xymatrix{\bullet \ar[r]\ar[rd]&\bullet \ar@<-2pt>[d] \ar@{-->}@<2pt>[d]^{\bZ} & \bullet \ar@{-->}[l]_{3} \ar@{-->}[r] & \bullet\\
&\bullet}$$
\caption{An example of a thread quiver}
\end{figure}

Every thread quiver $Q$ has an underlying quiver where there is no distinction between the standard and the thread arrows.  To avoid confussion, we will refer to this underlying quiver by $Q_r$.

Starting from a semi-hereditary dualizing $k$-variety, we will associate a thread quiver in the following way.

\begin{construction}\label{construction:MakeThreadQuiver}
Let $\aa$ be a semi-hereditary dualizing $k$-variety.  Let $\{ [X_i,Y_i] \}_{i \in I}$ be the set of all maximal threads in $\aa$.  The full subcategory of $\aa$ consisting of all objects which are not supported on $\bigcup_{i \in I}[X_i,Y_i]$ is called $\bb$.  By Proposition \ref{proposition:AllThreads}, this is again a semi-hereditary dualizing $k$-variety.  Proposition \ref{proposition:PathCategory} yields $\bb \cong kQ_r$ for a strongly locally finite quiver $Q_r$.

Accoring to Corollary \ref{corollary:ThreadsPosets}, every thread $[X_i,Y_i] \subset \ind \aa$ corresponds to a poset of the form $\bN \cdot (\TT \stackrel{\rightarrow}{\times} \bZ) \cdot -\bN$ where $\TT$ is a linearly ordered set.  We will replace one arrow from $X^- \to Y^+$ in $Q_r$ by $\xymatrix@1{X^- \ar@{-->}[r]^{\TT} & Y^-}$.
\end{construction}

\begin{example}
Let $\LL = \bN \cdot (\TT \stackrel{\rightarrow}{\times} \bZ) \cdot -\bN$, then the thread quiver associated with $k\LL$ is
$$\xymatrix@1{\bullet \ar@{-->}[r]^{\TT} & \bullet}$$
\end{example}

Given a thread quiver $Q$, we will construct an associated semi-hereditary finite $k$-variety.

\begin{construction}\label{construction:ThreadQuiver}
Let $Q$ be a thread quiver with underlying strongly locally finite quiver $Q_r$.  With every thread $t \in Q_t$, we denote by $f^t: k(\cdot \to \cdot) \to kQ_r$ the functor associated with the obvious embedding $(\cdot \to \cdot) \to Q_r$.
We define the functor
$$f: \bigoplus_{t \in Q_t} k(\cdot \to \cdot) \to kQ_r.$$

With every thread $t$, there is an associated linearly ordered set $\TT_t$.  We will write $\LL_t = \bN \cdot (\TT_t \stackrel{\rightarrow}{\times} \bZ) \cdot -\bN$.  Denote by
$$g^t: k(\cdot \to \cdot) \to k\LL_t$$
a chosen fully faithful functor given by mapping the extremal points of $\cdot \to \cdot$ to the minimal and maximal objects of $\LL$, respectively.  We will write
$$g: \bigoplus_{t \in Q_t} k(\cdot \to \cdot) \to \bigoplus_{t \in Q_t} k\LL_t.$$

We define the category $kQ$ as a 2-push-out of the following diagram.

$$\xymatrix{
\bigoplus_{t \in Q_t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}^{i}[d] \\
\bigoplus_{t \in Q_t} k\LL_t \ar@{-->}[r]_-{j} & kQ
}$$
\end{construction}

\begin{remark}
Given a thread quiver $Q$, Construction \ref{construction:ThreadQuiver} will only define $kQ$ up to equivalence.
\end{remark}

\begin{observation}
The functors $f^t$ have left adjoints (denoted by $f^t_L$) and right adjoints (denoted by $f^t_R$).  The induced functors
$$f_L, f_R : kQ_r \to \bigoplus_{t \in Q_t} k(\cdot \to \cdot)$$
are left and right adjoints for $f$, respectively.

Similarly, the functors $g_t$ have left adjoints (denoted by $g^t_L$) and right adjoints (denoted by $g^t_R$, giving rise to the functors
$$g_L, g_R : \bigoplus_{t \in Q_t} k\LL_t \to \bigoplus_{t \in Q_t} k(\cdot \to \cdot)$$
which are then left and right adjoints for $g$, respectively.
\end{observation}

\begin{proposition}
The functors $i$ and $j$ from Construction \ref{construction:ThreadQuiver} both have left and right adjoints.  Furthermore, $i$ is fully faithful and $j$ is faithful.
\end{proposition}

\begin{proof}
We start by showing $i$ has a left adjoint $i_L: kQ \to kQ_r$ as defined in Figure \ref{fig:LeftAdjointOfPsi}.  Consider the first diagram in Figure \ref{fig:LeftAdjointOfPsi}, where the natural transformation is given by
$$1_{f} \bullet \epsilon_g: f \stackrel{\sim}{\Rightarrow} f \circ g_L \circ g.$$
We can complete this diagram as shown in Figure \ref{fig:LeftAdjointOfPsi}.  We claim $i_L: \pp \to kQ_r$ is a left adjoint to $i$.  To prove this, we shall define a unit $\eta:  1_\pp \Rightarrow i \circ i_L$ and a counit 
$\epsilon: i_L \circ i \Rightarrow 1_{kQ_r}$ and show that
$$(1 \bullet \epsilon)\circ(\eta \bullet 1) = 1 \mbox{ and } (\epsilon \bullet 1)\circ(1 \bullet \eta) = 1.$$

\begin{figure}
	\centering
	\exa
	$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} \xtwocell[rrdd]{}\omit{^<0>}& {k Q_r} \ar@/^2pc/@{=}[rdd] \\
\bigoplus_{t} k\LL_t \ar@/_2pc/[rrd]_{f \circ g_L} \\
&& {k Q_r}}$$
	\exb
		$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} \xtwocell[rd]{}\omit{^<0>\alpha}& {k Q_r} \ar[d]^{i} \ar@/^2pc/@{=}[rdd] \xtwocell[rdd]{}\omit{<0>\gamma}\\
\bigoplus_{t} k\LL_t \ar[r]_-{j} \ar@/_2pc/[rrd]_{f \circ g_L} \xtwocell[rrd]{}\omit{^<0>\beta}& \pp\ar@{-->}[rd]_{i_L} \\
&& {k Q_r}}$$
   \exc
	\label{fig:LeftAdjointOfPsi}
\end{figure}

\begin{figure}
	\centering
	\exa
		$$\xymatrix@+20pt{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}[d]^{i} \ar@/^/[rdd]^{i} \\
\bigoplus_{t} k\LL_t \ar@{-->}[r]_-{j} \ar@/_/[rrd]_{j} & \pp\ar@{==}[rd] \\
&& {\pp}}$$
  \exb
		$$\xymatrix@+20pt{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}[d]^{i} \ar@/^/[rdd]^{i} \\
\bigoplus_{t} k\LL_t \ar@{-->}[r]_-{j} \ar@/_/[rrd]_{j \circ g \circ g_L} & \pp\ar@{-->}_{i \circ i_L}[rd] \\
&& {\pp}}$$
  \exc
	\caption{Construction of unit}
	\label{fig:UnitOfPsi}
\end{figure}

We define $\epsilon = \gamma^{-1}: i_L \circ i \Rightarrow 1_{kQ_r}$ with $\gamma$ as in the second diagram in Figure \ref{fig:LeftAdjointOfPsi}.  For the definition of $\eta$, consider the diagrams in Figure \ref{fig:UnitOfPsi}, where the natural transformations on the right-hand side are given by
\begin{eqnarray*}
1_{i} \bullet \gamma &:& i \Rightarrow i \circ i_L \circ i \\
(1_{i} \bullet \beta) \circ (\alpha \bullet 1_{g_L}) &:& j \circ g \circ g_L \Rightarrow i \circ f \circ g_L \Rightarrow i \circ i_L \circ j
\end{eqnarray*}
There is a modification, going from the 2-natural transformation on the left-hand side of Figure \ref{fig:UnitOfPsi} to the one on the right-hand side, given by
\begin{eqnarray*}
1_{i} &:& i \Rightarrow i \\
1_{j} \bullet \eta_g&:& j \Rightarrow j \circ g \circ g_L
\end{eqnarray*}
This modification corresponds to a natural transformation $\eta: 1_{\pp} \Rightarrow i \circ i_L$, giving the following commutative diagrams

$$\xymatrix@C+20pt@R+5pt{
i \ar@{=}[r]\ar@{=}[d] & i \ar@{=>}[d]^{1 \bullet \gamma} & {j} \ar@{=>}[r]^-{1 \bullet \eta_{g}} \ar@{=}[d] & {j \circ g \circ g_L}\ar@{=>}[d]^{(1_{i} \bullet \beta) \circ (\alpha \bullet 1_{g_L})} \\
i \ar@{=>}[r]_-{\eta \bullet 1} & {i \circ i_L \circ i} & {j} \ar@{=>}[r]_-{\eta \bullet 1} & i \circ i_L \circ j}$$

From the first commutative diagram, we obtain
$$(1 \bullet \epsilon)\circ(\eta \bullet 1) = (1 \bullet \gamma)^{-1}\circ(\eta \bullet 1) = 1.$$

\begin{figure}
	\centering
	\exa
		$$\xymatrix@+0pt{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}[d]^{i} \ar@{=}@/^/[rrddd] \\
\bigoplus_{t} k\LL_t \ar@{-->}[r]_-{j} \ar@/_/[rrrdd]_{f \circ g_L} & \pp\ar@{==}[rd] \\
&& {\pp} \ar[rd] \\
&&& kQ_r}$$
  \exb
		$$\xymatrix@+0pt{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}[d]^{i} \ar@/^/[rrddd]^{i \circ i} \\
\bigoplus_{t} k\LL_t \ar@{-->}[r]_-{j} \ar@/_/[rrrdd]_{f \circ g_L \circ g \circ g} & \pp\ar[rd]_{i \circ i_L} \\
&& {\pp} \ar[rd] \\
&&& kQ_r}$$
  \exc
	\caption{2nd equation}
	\label{fig:2ndEquation}
\end{figure}

To show the other equation, and establish the adjointness of $i$ and $i_L$, we add the functor $i_L: \pp \to k Q_r$ to the diagrams in Figure \ref{fig:UnitOfPsi} (see Figure \ref{fig:2ndEquation}).  The natural transformations of the second diagram of Figure \ref{fig:2ndEquation} are given by
\begin{eqnarray*}
(1 \bullet \delta) \circ (\beta \bullet 1) &:&  f \circ g_L \circ g \circ g_L \Rightarrow i_L \circ j \circ g \circ g_L \Rightarrow i_L \circ i \circ i_L \circ j\\
1 \bullet \gamma \bullet 1 &:& i_L \circ i \Rightarrow i_L \circ i \circ i_L \circ i
\end{eqnarray*}

It is easily verified that the modification $\Lambda$ given by
\begin{eqnarray*}
1 \bullet 1 \bullet \eta_{g}&:& f \circ g_L \Rightarrow f \circ g_L \circ g \circ g_L \\
\gamma &:& 1_{kQ_r} \Rightarrow i_L \circ i
\end{eqnarray*}
corresponds to the natural transformation $1 \bullet \eta: i_L \rightarrow i_L \circ i \circ i_L$.

\begin{figure}
	\centering
		$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {k Q_r} \ar@{-->}[d]^{i} \ar@{=}@/^3pc/[rrrdddd] \\
\bigoplus_{t} k \LL_t \ar@{-->}[r]_-{j} \ar@/_5pc/[rrrrddd]_{f \circ g_L \circ g_R \circ g_L} \ar@{-->}[r]_-{j} \ar@/_3pc/[rrrrddd]^{f \circ g_L} \xtwocell[rrrrddd]{}\omit{^<10>} & \pp\ar[rd] \\
&& kQ_r \ar[rd] \ar@{=}@/^2pc/[rrdd] \xtwocell[rrdd]{}\omit{^<-3>\epsilon} \\
&&& \pp \ar[rd]\\
&&&& kQ_r}$$
	\caption{Proof of adjointness}
	\label{fig:PsiAdjoint2}
\end{figure}

Likewise, the modification $\Omega$ (shown in Figure \ref{fig:PsiAdjoint2}) given by
\begin{eqnarray*}
1 \bullet \epsilon_{g} \bullet 1&:& f \circ g_L \circ g \circ g_L \Rightarrow f \circ g_L \\
\epsilon &:& i_L \circ i \Rightarrow 1_{kQ_r}
\end{eqnarray*}
corresponds to the natural transformation $\epsilon \bullet 1: i_L \circ i \circ i_L \rightarrow i_L$.  Since $\Omega \circ \Lambda = 1$, we find
$$(\epsilon \bullet 1)\circ(1 \bullet \eta) = 1.$$
We conclude $i_L$ is indeed left adjoint to $i$.

Similarly, one verifies that the functor $i_R$, defined in Figure \ref{fig:RightAdjointOfPsi}, is a right adjoint to $i$.  For the left and right adjoint to $j$, we consider the functors $j^s_L$ and $j^s_R$ given by the diagrams in Figure \ref{fig:AdjointsOfPhi}.  The left and right adjoints to $j$ are then given by $\bigoplus_s j^s_L$ and $\bigoplus_s j^s_R$, respectively.

\begin{figure}
	\centering
$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} \xtwocell[rd]{}\omit{^<0>\alpha}& {k Q_r} \ar[d]^{i} \ar@/^2pc/@{=}[rdd] \xtwocell[rdd]{}\omit{<0>\gamma}\\
\bigoplus_{t} k\LL_t \ar[r]_-{j} \ar@/_2pc/[rrd]_{j \circ g_R} \xtwocell[rrd]{}\omit{^<0>\beta}& \pp\ar@{-->}[rd]_{i_R} \\
&& {k Q_r}}$$
 \caption{Construction of $i_R$}
 \label{fig:RightAdjointOfPsi}
\end{figure}

\begin{figure}
	\centering
	\exa
		$$\xymatrix{
\bigoplus_{t} k(\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {kQ_r} \ar[d]^{i} \ar@/^2pc/[rdd]^{g^s \circ j^s_L} \\
\bigoplus_{t} k\LL_t \ar[r]_-{j} \ar@/_/[rrd]_{\pi_s} & kQ \ar@{-->}[rd]^{j^s_L} \\
&& k\LL_s}$$
  \exb
  $$\xymatrix{
\bigoplus_{t} k(\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {kQ_r} \ar[d]^{i} \ar@/^2pc/[rdd]^{g^s \circ f^s_R} \\
\bigoplus_{t} k\LL_t \ar[r]_-{j} \ar@/_/[rrd]_{\pi^s} & kQ \ar@{-->}[rd]^{j^s_R} \\
&& k\LL_s}$$
  \exc
	\caption{The definition of $j_L$}
	\label{fig:AdjointsOfPhi}
\end{figure}

To show $i$ is indeed fully faithful, it suffices to remark that $i_L\circ i$ is naturally equivalent to the identity.  Similarly, we have that $j^s_L\circ j^s$ is naturally equivalent to the identity, for each $s \in Q_t$ so that $j$ is faithful.
\end{proof}

\begin{example}\label{example:NotFull}
Let $Q$ be one of the thread quivers given in Figure \ref{fig:NotFull}, then the functor $j$ is not full.
\end{example}

\begin{figure}
	\centering
		\exa
		$$\xymatrix{&& \\ \ar@{-->}[r]&\ar@{-->}[r]\ar[u]&}$$
		\exb
		$$\xymatrix{& \\ \ar@{-->}[ru] \ar@{-->}[rd] \\ &}$$
		\exc
	\caption{Thread quivers from Example \ref{example:NotFull}}
	\label{fig:NotFull}
\end{figure}

\begin{example}
Let $Q$ be the thread quiver given by
$$\xymatrix@1{\cdot \ar@{-->}[r]^{\LL} & \cdot}$$
The associated finite $k$-variety equivalent to $k(\bN \cdot \LL \stackrel{\rightarrow}{\times} \bZ \cdot -\bN)$.
\end{example}

Although Construction \ref{construction:ThreadQuiver} will not yield all (semi-hereditary) finite $k$-varieties, the following theorem says it is general enough to give all semi-hereditary dualizing $k$-varieties.

\begin{proposition}\label{proposition:kQIsGood}
If $Q$ is a thread quiver with $Q_r$ strongly locally finite, then $kQ$ is a semi-hereditary dualizing $k$-variety.
\end{proposition}

\begin{proof}
First note that $\mod kQ$ is naturally embedded into $\mod kQ_r \oplus \mod \LL$.  Since the latter category is Ext-finite, so is the former.  In particular, $kQ$ is Hom-finite.  It follows easily from \ref{} that idempotents split, such that $kQ$ is a finite $k$-variety.

To show that $kQ$ is semi-hereditary (thus that $\mod kQ$ is abelian and hereditary) it suffices to show that the kernel between finitely generated projectives of $\Rep kQ$ is projective and splits off.

A finitely generated projective module $kQ(-,A) \in \Mod kQ$ corresponds to a diagram
$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} \xtwocell[rd]{}\omit{^<0>\alpha}& {k Q_r} \ar[d]^{i} \ar@/^2pc/[rdd]^{kQ_r(-,i_R A)} \xtwocell[rdd]{}\omit{<0>\gamma}\\
k\LL \ar[r]_-{j} \ar@/_2pc/[rrd]_{\LL(-,j_R A)} \xtwocell[rrd]{}\omit{^<0>\beta}& kQ\ar@{-->}[rd]_{kQ(-,A)} \\
&& \Mod k}$$
This shows that the natural embedding $\Mod kQ \to \Mod kQ_r \oplus \Mod k\LL$ restricts to an embedding $\mod kQ \to \mod kQ_r \oplus \mod k\LL$.

Let $kQ(-,A) \to kQ(-,B)$ be a map between finitely generated projectives.  Since $\mod kQ_r$ and $\mod k\LL$ are hereditary, we get the exact sequences
$$\xymatrix@1{0 \ar[r]& kQ(-,K_1) \ar[r] & kQ(-,i_R A) \ar[r]& kQ(-,i_R B)}$$
and
$$\xymatrix@1{0 \ar[r]& k\LL(-,K_2) \ar[r] & k\LL(-,j_R A) \ar[r]& k\LL(-,j_R B)}$$
where the kernels split off.

These exact sequences induce the following commutative diagram
$$\xymatrix{0 \ar[r]& \aa(f-,K_1)\ar@{-->}[d] \ar[r] & \aa(f-,i_R A) \ar[d]\ar[r]& \aa(f-,i_R B) \ar[d]\\
0 \ar[r]& \aa(g-,K_2) \ar[r] & \aa(g-,j_R A) \ar[r]& \aa(g-,j_R B)}$$
which shows that the kernel of $kQ(-,A) \to kQ(-,B)$ splits off, and hence is projective.  We have shown $kQ$ is semi-hereditary.

We proceed to show $kQ$ is a dualizing $k$-variety, thus that $D: \mod kQ \to \mod kQ^\circ$ is a duality.  Consider the diagram below
$$\xymatrix{
\bigoplus_{t} k (\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} \xtwocell[rd]{}\omit{^<0>\alpha}& {k Q_r} \ar[d]^{i} \ar@/^2pc/[rdd]^{kQ_r(-,i_R A)} \xtwocell[rdd]{}\omit{<0>\gamma}\\
k\LL \ar[r]_-{j} \ar@/_2pc/[rrd]_{\LL(-,j_R A)} \xtwocell[rrd]{}\omit{^<0>\beta}& kQ\ar@{-->}[rd]_{kQ(-,A)} \\
&& \Mod k}$$
where $N$ and $L$ are now contravariant functors, and $\alpha$ natural equivalence.  The functors $DN \in \mod kQ_r$ and $DL \in \mod \LL$ are covariant, giving rise to a covariant functor $M: kQ \to \mod k$. Again applying $D$ and using $D^2 \cong 1$ and that $kQ_r$ and $\LL$ are dualizing $k$-varieties yields the result.
\end{proof}

\begin{theorem}
Let $\aa$ be a semi-hereditary dualizing $k$-variety, then $\aa$ may be obtained by Construction \ref{construction:ThreadQuiver} from a thread quiver $Q$, where $Q$ is strongly locally finite.
\end{theorem}

\begin{proof}
It has been established in Proposition \ref{proposition:kQIsGood} that $kQ$ is indeed a semi-hereditary dualizing $k$-variety, so that we need only to show every semi-hereditary dualizing $k$-variety arises in this way (up to equivalence).

Let $\aa$ be a semi-hereditary dualizing $k$-variety and $Q$ be the corresponding thread quiver, as in Construction \ref{construction:MakeThreadQuiver}.  The functors $i_\aa: kQ_r \to \aa$ and from $j_\aa: k\LL \to \aa$ give rise to a diagram as in Figure \ref{fig:DefinitionOfF}.

\begin{figure}
  $$\xymatrix{
\bigoplus_{t} k(\cdot \to \cdot) \ar[r]^-{f} \ar[d]_{g} & {kQ_r} \ar[d]^{i} \ar@/^2pc/[rdd]^{i_\aa} \\
\bigoplus_{t} k\LL_t \ar[r]_-{j} \ar@/_/[rrd]_{j_\aa} & kQ \ar@{-->}[rd]^{F} \\
&& \aa}$$
	\caption{The definition of the functor $F: kQ \to \aa$}
	\label{fig:DefinitionOfF}
\end{figure}

It is easy to check that this functor $F: kQ \to \aa$ is essentially surjective; we will continue by showing $F$ is also fully faithfull by proving $kQ(X,-) \cong \aa(FX,F-)$ for all $X\in \Ob kQ$.

Using the equivalence $(-\circ \sigma)$, the functor $\aa(FX,F-)$ induces a functor $\aa(FX,F \circ i -) \oplus \aa(FX,F \circ i -): kQ_r \oplus k\LL \to \mod k$.  We find
\begin{eqnarray*}
\aa(FX,F \circ i -) \oplus \aa(FX,F \circ i -) &\cong& \aa(FX,i -) \oplus \aa(FX,j -) \\
&\cong& kQ_r(i_L \circ FX, -) \oplus k\LL(j_L \circ FX, -) \\
&\cong& kQ_r(i_L X, -) \oplus k\LL(j_L X,-),
\end{eqnarray*}
which is isomorphic to $(-\circ \sigma)\left(kQ(X,-)\right)$.  We have shown that $F: kQ \to \aa$ is fully faithfull, and hence also an equivalence.
\end{proof}

\begin{proposition}\label{proposition:TiltingArms}
Let $Q$ be a thread quiver and let $\{\alpha_i: \xymatrix@1{X_i \ar@{-->}[r] & Y_i}\}$ be a set of thread arrows of $Q$ such that each $Y_i$ is a sink and such that $\alpha_i$ is the only arrow ending in $Y_i$.  Define $Q'$ to be the thread quiver obtained by removing the vertices $Y_i$ and replacing each $\alpha_i: \xymatrix@1{X_i \ar@{-->}[r] & Y_i}$ by an $A_\infty$-quiver with zig-zag orientation.  The categories $\rep Q$ and $\rep Q'$ are derived equivalent.
\end{proposition}

\begin{proof}
There is a straightforward map from the indecomposable projectives of $\rep Q'$ into $\Db \rep Q$ lifting to a fully faithful map $i: \Db \rep Q' \to \Db \rep Q$.  Note that $i$ commutes with the Serre functor, because it commutes with the Serre functor on generators.

To show that $i$ is essentially surjective, we need only to show each $kQ(-,Y_i)$ lies in the essential image of $i$.  However
\end{proof}

\begin{example}
\end{example}

\begin{remark}
It follows from the construction of a semi-hereditary dualizing $k$-variety $\aa$ from a thread quiver $Q$ (Construction \ref{construction:ThreadQuiver}) that, up to isomorphism, every $k$-representation of $\aa$ is given by
\begin{enumerate}
\item a representation $M(-):kQ_r \to \mod k$ of $kQ_r$,
\item for every thread $t$, a representation $N_t(-):\LL_t \to \mod k$, and
\item a natural equivalence $\alpha: M(f-) \Rightarrow N(g-)$.
\end{enumerate}
\end{remark}

\begin{proposition}
Let $\aa$ be a semi-hereditary dualizing $k$-variety.  Let $\{\aa_i\}_i$ be the filtered system of all subcategories of $\aa$ such that $\ind \aa_i$ is finite.  There is an equivalence
$$2\lim\limits_{\stackrel{\rightarrow}{i}} \mod \aa_i \cong \mod \aa.$$
\end{proposition}
